Electronic schematic for bio-plausible dopamine neuromodulation of eSTDP and iSTDP

In this technical report we present novel results of the dopamine bio-plausible neuromodulation excitatory (eSTDP) and inhibitory (iSTDP) learning. We present the principal schematic for the neuromodulation of D1 and D2 receptors of dopamine, wiring schematic for both cases as well as the simulatory experiments results done in LTSpice.

==> _writingarticle.tex <==
writing article
% https://cseweb.ucsd.edu/~wgg/CSE210/howtoread.html
% https://ceprofs.civil.tamu.edu/ssocolofsky/downloads/paper_how-to.pdf
%
%
%
% 2 Before starting to write
% Before you start to write, you should spend some time thinking about the article content. At this stage, you should write down ideas in a free form, creating a general outline for the paper. Jirka suggests you consider such questions as:
% •What is the message of the paper?
% •What is the new result or contribution that you want to describe?
% •What do you want to convince people of?
% If you have not already done so, you should conduct a thorough literature search to identify those important contributions that are related to your work. As you are ready to submit your article, it is always helpful to do one more search; including articles that were published just as you submit your paper will show that you are aware of the current work going on in your ﬁeld (Russel & Morrison 2003).
% As you get ready to write, try to summarize these initial ideas into concrete bullets that will eventually become paragraphs. Start to organize these bullets into a logical structure and develop them in the form of key sentences. If the outline is convincing, then the article will be successful. Likewise, a weak outline cannot be saved by any good writing skills.
%
%
%
% 3 Structure and function of the article: What to write
% In formulating the outline it is important to know that most engineering or science journal articles have a well-accepted general format. Each of the following sections are included, usually also in this order, though speciﬁc articles may disguise them under diﬀerent section titles that relate closer to the actual contents of each section. These sections are
% 1.Abstract
% 2.Introduction
% 3.Methods
% 4.Results
% 5.Discussion
% 6.Summary and Conclusions
% 7.Acknowledgments
% 8.References
% Each part serves a diﬀerent purpose and has a narrowly deﬁned content and purpose. Understanding how each section functions together with the whole will help the author minimize overlap and repetition.

% 3.1 The Abstract
% The abstract is a single paragraph that precedes the article and summarizes the content. The abstract reduces the whole paper to a single paragraph. Many times, the abstract will be published by itself in an index to the article and often only the words in the abstract can be searched using library databases; hence, the abstract is a critical element of the research paper. It contains a general introduction to the topic, outlines the major results, and summarizes the conclusions. It is shorter than the summary and conclusions section of the main paper and is less of an outline than the closing paragraph of the introduction. Often, the abstract does not require citations; some journals discourage use of mathematical symbols. The guideline for a good abstract is:
% The abstract should inform the reader in a succinct manner as to what the article is about and what the major contributions are that are discussed
% The abstract is more general than the conclusions section and can have a staccato literary style.
% The following are two examples of well-written abstracts:
% • “Fishes swim by ﬂapping their tail and other ﬁns. Other sea creatures, such as squid and salps, eject ﬂuid intermittently as a jet. We discuss the ﬂuid mechanics behind these propulsion mechanisms and show that these animals produce optimal vortex rings, which give the maximum thrust for a given energy input. We show that ﬁshes optimize both their steady swimming eﬃciency and their ability to accelerate and turn by producing an individual optimal ring with each ﬂap of the tail or ﬁn. Salps produce vortex rings directly by ejecting a volume of ﬂuid through a rear oriﬁce, and these are also optimal. An important implication of this paper is that the repetition of vortex production is not necessary for an individual vortex to have the ‘optimal characteristics.” (Linden & Turner 2004).
% • “Aquatic plants convert mean kinetic energy into turbulent kinetic energy at the scale of the plant stems and branches. This energy transfer, linked to wake generation, aﬀects vegetative drag and turbulence intensity. Drawing on this physical link, a model is developed to describe the drag, turbulence and diﬀusion for ﬂow through emergent vegetation which for the ﬁrst time captures the relevant underlying physics, and covers the natural range of vegetation density and stem Reynolds numbers. The model is supported by laboratory and ﬁeld observations. In addition, this work extends the cylinder-based model for vegetative resistance by including the dependence of the drag coeﬃcient, CD, on the stem population density, and introduces the importance of mechanical diﬀusion in vegetated ﬂows.” (Nepf 1999).
% Both abstracts tell the reader what to expect, summarize what the important contribution is, and entice the reader to look further. Neither abstract gives detailed quantitative results. This level of detail lets the reader know what to expect without overwhelming him with details, derivations, or sophisticated results—the reader is equipped to safely set the article aside or delve deeper to uncover the details.



% 3.2 The Introduction
% The introduction is perhaps the most important sections in a research article. Nearly every reader will at least skim through the introduction. The introduction is also written with the strictest requirements in terms of organization.

% 3.2.1 Paragraph 1
% The ﬁrst paragraph should follow the inverted triangle principle: start with a broad statement and become more detailed until ﬁnally identifying the speciﬁc problem that the paper addresses. The purpose of the ﬁrst paragraph is to interest the reader in the paper, to clearly identify for the reader what the paper will address, and to quickly bring the reader to the edge of knowledge in the ﬁeld the paper addresses (Russel & Morrison 2003). The paragraph should end with the general problem addressed by the paper.
% To have the greatest impact, the ﬁrst sentence should be broad in scope and should attract the reader’s attention. Here are ﬁve opening sentences from the current issue of the Journal of Fluid Mechanics:
% •“Turbulence is not a universal state of nature, but there are similar forms of eddy motion, and mixing processes with similar statistical properties for a variety of turbulent ﬂows within a particular ‘type.” (Hanazaki & Hunt 2004).
% •“There is a long-standing interest in ﬂow over isolated topography, such as seamounts, with regard to both theoretical and practical issues.” (Nycander & Lacasce 2004).
% •“Breaking waves at the sea surface promote vigorous mixing of momentum, energy, and scalars, and thus are a key process in upper-ocean dynamics and air-sea interaction.” (Sullivan et al. 2004).
% •“We investigate a family of exact solutions of the Navier-Stokes equations that describe the steady ﬂow of a rivulet down an incline.” (Perazzo & Gratton 2004).
% •“Granular ﬂow exhibits a variety of dynamical phenomena, which have been attracting research interest for many years (for reviews, see e.g. Savage 1984 and Jaeger, Nagel & Behringer 1996).” (Mitarai & Nakanishi 2004).
% Clearly, there is a wide variety of levels of detail, but each statement, except for the fourth example, follows the rule of thumb outlined above
% Start with an attention-getting broad statement that establishes a general topic for the article
% Here are four more examples from papers by some of the best authors:
% •“Observations of swimming ﬁshes and other organisms such as salps reveal a series of vortex rings forming behind the animals, which play an important part in their mechanisms of propulsion.” (Linden & Turner 2004).
% •“Freshwater and saltwater wetlands provide important transition zones between terrestrial and aquatic systems, mediating exchanges of sediment [Phillips, 1989], nutrients [Nixon, 1980; Barko et al., 1991], metals [Orson et al., 1992; Lee et al., 1991], and other contaminants [Dixon and Florian, 1993].” (Nepf 1999).
% •“Shallow ﬂows are ubiquitous in nature” (Jirka 2001).
% •“The entrainment hypothesis was ﬁrst introduced by Sir Goeﬀrey Taylor in a wartime report on the dynamics of hot gases rising in air.” (Turner 1986).
% •“The convection currents which rise from heated bodies have been discussed previously, but in most cases attention has been directed towards ﬁnding the distribution of ﬂuid velocity and temperature near such bodies.” (Morton et al. 1956).
% These also exhibit a wide variety, but each follows our general principle.
% The next sentences of the introduction narrow the topic. These sentences often contain citations to other work and build up to a speciﬁc lack of knowledge that culminates in the problem statement. This section can vary in length from one to many sentences, but the general goal is to educate the reader about an important gap in knowledge that the paper will address (Russel & Morrison 2003). Here are three good examples of a complete introductory paragraph: the ﬁrst is short, the second contains no citations, and the third is longer. The problem statement in each paragraph has also been italicized.
% •“There is a long-standing interest in ﬂow over isolated topography, such as seamounts, with regard to both theoretical and practical issues. Trapped ﬂows are often observed over seamounts, and these ﬂows evidently aﬀect the distribution and concentration of subsurface fauna, ﬁlter feeders and the like (e.g. Genin, Noble & Lonsdale 1989 and references therein). These ﬂows are often so intense that they alter the ambient vorticity and, as such, can modify the allowable frequencies of internal waves. This in turn may aﬀect wave breaking (Kunze & Toole 1997 and references therein).” (Nycander & Lacasce 2004), emphasis added.
% •“Observations of swimming ﬁshes and other organisms such as salps reveal a series of vortex rings forming behind the animals, which play an important part in their mechanisms of propulsion. Fishes produce these vortices by an undulatory motion of the body and tail, controlling the periodic shedding of vorticity into the wake, and salps form them more directly, by ejecting ﬂuid backwards through an oriﬁce. In both cases the vortices roll up into three-dimensional (3D) ring-like structures. For ﬁshes, the important question is what frequency and amplitude of the undulatory motion provide the most eﬃcient propulsion? A similar question faces the oarsman of a gondola. For eﬃcient motion, should the oar be moved slowly at large amplitude or quickly with a smaller amplitude? Here, we discuss this question, not in terms of a periodic motion, but by considering each ﬂap of the tail or ﬁn as a single event. This may be repeated periodically during steady swimming, but may be aperiodic during a turn or other manoeuvre. For other organisms using a jet for propulsion, the question is how long a jet provides the optimal eﬃciency.” (Linden & Turner 2004), emphasis added.
% •“Granular ﬂow exhibits a variety of dynamical phenomena, which have been attracting research interest for many years (for reviews, see e.g. Savage 1984 and Jaeger, Nagel & Behringer 1996). Its complex behavior can be seen even in a simple situation like the gravitational ﬂow on a slope. When the inclination angle is large and the slope is rough, a rapid and relatively low-density ﬂow is realized, and the interaction between grains is dominated by inelastic collisions. On the other hand, when the inclination angle is small, the ﬂow becomes dense and slow, and the frictional interaction plays an important role (Savage 1984; Mitarai & Nakanishi 2003). The comprehensive rheology of the granular ﬂow has not been fully understood yet, except for the rapid collisional ﬂow regime, where hydrodynamic models have been developed with constitutive relations based on the kinetic theory of inelastic hard spheres (Jenkins & Savage 1983; Campbell 1990; Lun et al. 1984; Goldhirsh 2003); it has been demonstrated that some quantitative agreement can be achieved for the steady ﬂow by introducing the spinning motion of each grain (Mitarai, Hayakawa & Nakanishi 2002). The steady granular ﬂow, however, turns out to be unstable in various ways, and shows rich phenomena.” (Mitarai & Nakanishi 2004), emphasis added.
% In each case there is reference to broader knowledge beyond the scope of the actual article. This knowledge is narrowed to a speciﬁc problem, or gap, in the understanding of the subject. As a result, each example illustrates our next rule-of-thumb (adapted from Russel & Morrison (2003)):
% Narrow the topic in successive sentences that outline the state of the art and introduce a gap in knowledge
% Each paragraph also contains a statement of the main problem addressed by the article. The second example has a speciﬁc problem statement, though it is expanded in the ﬁnal sentence. The other two paragraphs have somewhat more open-ended problem statements. This statement is not always the ﬁnal sentence; however, any statements that follow the problem statement serve to make it more speciﬁc or further justify its importance. Our ﬁnal rule for the introductory paragraph follows:
% End the introductory paragraph with a general statement of the problem and optional supporting/specifying statements
% By following this procedure, the introductory paragraph will serve its purpose of attracting the reader, identifying the context of the problem, and specifying the general direction of the article. After reading this paragraph, the reader should be able to safely set aside the article if he concludes that the topic is not applicable to his area of research. Hence, the statement of the problem should be speciﬁc enough for the reader to anticipate the kinds of results that will be reported. Writing in this way, your article will be read by more people and not overlooked by your colleagues in the ﬁeld.

% 3.2.2 Middle paragraphs
% Following the introductory paragraph is a series of paragraphs that traditionally function as a literature review (McNown 1996b). The extent of this section varies somewhat by journal and by topic, but generally follows a speciﬁc format. The beginning of the literature review should cite the most important historical contributions that build the foundation to the topic the paper will extend (Russel & Morrison 2003). The goal is not to cite everything, as in a review article, but to cite the seminal contributions that directly lead to the problem the article addresses. The remaining paragraphs should focus on the state-of-the-art knowledge base and the signiﬁcant diﬀerences between what has already been published and the new contribution that your article is presenting. Together, these paragraphs give another guiding principle:
% The literature review identiﬁes the seminal historical contributions, outlines the state of knowledge, and justiﬁes the novelty of the article’s contribution
% The literature review should be based on refereed journal articles to the extent possible. Conference proceedings can be referenced where they never resulted in journal publications; web sites can be referenced where they present unique, multi-media oriented content. Keep in mind that non-refereed material does not bolster an argument. Hence, the literature review gives credit to our predecessors and justiﬁes the need and novelty of the article’s contribution.

% 3.2.3 Final paragraph
% The introduction ends with the “road-map” paragraph. This paragraph outlines the remaining sections of the paper. It can either give a general outline of the contribution, or a speciﬁc, section-by-section breakdown of the remaining article. Here are two examples illustrating these two possibilities:
% •“In addition to the theory, we present results from numerical simulations. These are done in order to examine whether the predicted stable ﬂows can arise naturally as a result of the time-dependent evolution. As the initial condition, we use various non-stationary vortices near or on top of a seamount. We also revisit two-dimensional turbulence over a bump. The simulations are broadly supportive of the theoretical predictions, although time-dependence can produce exotic and interesting ﬁnal states.” (Nycander & Lacasce 2004).
% •“Section 2 introduces models for drag, turbulence, and diﬀusivity for ﬂow through emergent vegetation. Laboratory and ﬁeld experiments described in section 3 provide observations which support these models. The comparison of model prediction and experimental observation is given in section 4. Finally, the models are used to compare the mean ﬂow, turbulence intensity, and diﬀusivity in vegetated and unvegetated regions (section 5).” (Nepf 1999).
% This paragraph serves two important functions. First, it puts the complete contribution of the article in the context of the previous contributions, thereby, emphasizing novelty and the extent of the new contribution. Second, it guides the expert reader, who may want to skip sections of your article, to the sections that interest him. Thus, we have our ﬁnal principle for the Introduction:
% End the introduction by outlining for the reader the speciﬁc contribution of the article and tell the reader the overall organization
% This paragraph will also help you organize your logic: if this paragraph is unclear, the rest of the paper will be built on a weak foundation.

% 3.3 The Methods
% The methods sections often come disguised with other article-speciﬁc section titles, but serve a uniﬁed purpose: to detail the methods used in an objective manner without introduction of interpretation or opinion (van Wagenen 1990). The methods sections should tell the reader clearly how the results were obtained. They should be speciﬁc. They should also make adequate reference to accepted methods and identify diﬀerences. The governing principle is as follows:
% Describe all of the techniques used to obtain the results in a separate, objective Methods section
% In the case of a paper that develops both an analytical model and laboratory results, it is common to write separate methods sections for each. At the conclusion of the methods sections, the reader should be able to form an educated opinion about the quality of the results to be presented in the remaining sections (van Wagenen 1990).
% Here are ﬁve examples of the titles of the methods sections in some of the papers referenced above:
% •“2. Model Development; 2.1 Draft Model for Emergent Vegetation, 2.2 Turbulence Intensity within Emergent Vegetation, 2.3 Diﬀusion within Emergent Vegetation. 3. Methods; 3.1 Laboratory Experiments, 3.2 Field Experiments.” (Nepf 1999).
% •“Gravitational Convection; The main assumptions.” (Morton et al. 1956).
% •“2. Classiﬁcation of 2-D coherent structures in shallow ﬂows. 3. Methods of investigation.” (Jirka 2001).
% •“2. Theory of Vortex Ring Formation” (Linden & Turner 2004).
% •“2. Theory; 2.1. Conservation laws and variational principle, 2.2. Flat topography or circular seamount, 2.3. Irregular seamount, 2.4. Comparison with the theory of Carnevale & Frederiksen.” (Nycander & Lacasce 2004).
% One thing to notice is that subsections should only be used when there will be more than one subsection; a subsection implies that the material should be classiﬁed into more than one group.


% 3.4 The Results
% The results section and the following discussion section allow the most ﬂexibility in terms of organization and content. In general, the pure, unbiased results should be presented ﬁrst without interpretation (van Wagenen 1990). These results should present the raw data or the results after applying the techniques outlined in the methods section. The results are simply results; they do not draw conclusions. Often the results are combined with the discussion section, which does make interpretations and suggest implications. When these are presented in one section, there should be a clear distinction between a result and discussion. This could be done by paragraphing, by section headings, or by careful writing within a single paragraph. The main purpose of the results section, however, is to provide the data from your study so that other researchers can draw their own conclusions and understand fully the basis for your conclusions.
% A common format for the results section is to present a series of ﬁgures and to describe the ﬁgures in detail through the text. A good results section presents clear ﬁgures with eﬃcient text. The ﬁgures should support the assertions in the paper or illustrate the new insights. Where applicable, results should be illustrated in terms of non-dimensional variables. These characteristics lead to our principle for results sections:
% Results should be clear, convincing, and general and should be free from interpretations or opinions
% Whether together with the discussion or in their own section, results need to be communicated objectively.

% 3.5 The Discussion
% The discussion section is where the article interprets the results to reach its major conclusions. This is also where the author’s opinion enters the picture (van Wagenen 1990)—the discussion is where the argument is made. Often writers will combine the discussion and results sections so that they can avoid repetition and so that they can give their conclusions parallel with the results. This is acceptable if there maintains a clear distinction between facts and opinion. Most scientiﬁc papers, however, require the results and discussion to be in separate sections.
% A common feature of the discussion section is comparison between measured and modeled data or comparison among various modeling methods. Jirka suggests considering the following questions:
% • How do the results compare with earlier work?
% • What is new and signiﬁcant?
% Another common element in a discussion section applies the results obtained to solve a speciﬁc engineering or scientiﬁc problem. Some journals, notably the Journal of Hydraulic Engineering, even require a separate applications section for this purpose. The main feature of the discussion section can be summarized as follows:
% Discussion sections interpret the results to reach the main conclusions of the article
% The discussion section is the main impact section where the researcher has the most freedom to tout the implications of his research. A word of warning, though: never make an assertion of which you are not 100% sure—do not open the door for a negative review or the eventual rejection of your article. As a rule, it is better to be conservative. Most of the experts reading your article will draw their own conclusions anyhow. This section allows you to highlight the conclusions you think are important.


% 3.6 The Summary and Conclusions
% The ﬁnal section of the paper does not introduce any new information or insights: it merely summarizes and concludes. This section is longer than the abstract and generally includes more speciﬁc conclusions. It is often more quantitative than the abstract, however, listing equations or citations should not be necessary (McNown 1996a). The summary and conclusions section also has a more ﬂuid literary style than the abstract.
% A good format for this section is to write it in two paragraphs. The ﬁrst paragraph summarizes various sections of the article. The second paragraph draws the important conclusions. The summary paragraph is diﬀerent than that at the end of the introduction section. Here, the summary paragraph draws on the fact that the reader knows all of the new results presented in the article. It then summarizes what the important results where. The conclusion paragraph identiﬁes the signiﬁcant conclusions. McNown (1996a) suggests two possible formats for this second paragraph:
% 1. Organize based on logical ﬂow for points that are interconnected
% 2. Organize based on merit, where the most important items appear ﬁrst
% It is important to remember that this paragraph should not present new information. It may combine parts of the article to underscore an important conclusion, but it cannot present information that could not be gleaned from the other sections. A third, optional, paragraph may identify future research directions that ﬂow naturally from the article.
% The guiding principle for the summary and conclusions section may be formulated as follows:
% The summary and conclusions section tells the reader what has already been read and draws the important conclusions—keep it short and make it as speciﬁc as possible
% If the reader wants to know speciﬁcally what aspects of a problem your paper will address, he will often read the introduction and then the summary and conclusions section. Hence, it is important that all of the signiﬁcant ﬁndings are summarized and united in the signiﬁcant conclusions. Follow these guidelines and your papers will have maximum impact and receive the most positive reviews that your work warrants.


% 3.7 The Acknowledgments
% The acknowledgments are given at the end of the research paper and should at a minimum name the sources of funding that contributed to the article. You may also recognize other people who contributed to the article or data contained in the article, but at a level of eﬀort that does not justify their inclusion as authors.
% There is a growing trend to also acknowledge the contributions of the reviewers. This is a controversial issue. Since acknowledgment sections cannot be referenced or listed on a curriculum vitae, this seems only a means of getting the reviewers to agree with a revision and accept the paper. I would suggest that if the reviewer’s comments are great enough that they substantially changed the paper, the reviewer might be invited as an author; a ﬂowery acknowledgment seems unjustiﬁed, given that every article is presumed to have beneﬁted from reviewer comments.
